Entropically Patchy Particles: Engineering Valence through Shape Entropy

Patchy particles are a popular paradigm for the design and synthesis of nanoparticles and colloids for self-assembly. In "traditional" patchy particles, anisotropic interactions arising from patterned coatings, functionalized molecules, DNA, and other enthalpic means create the possibility for directional binding of particles into higher-ordered structures. Although the anisotropic geometry of non-spherical particles contributes to the interaction patchiness through van der Waals, electrostatic, and other interactions, how particle shape contributes entropically to self-assembly is only now beginning to be understood. It has been recently demonstrated that, for hard shapes, entropic forces are directional. A newly proposed theoretical framework that defines and quantifies directional entropic forces demonstrates the anisotropic--that is, patchy--nature of these emergent, attractive forces. Here we introduce the notion of entropically patchy particles as the entropic counterpart to enthalpically patchy particles. Using three example "families" of shapes, we judiciously modify entropic patchiness by introducing geometric features to the particles so as to target specific crystal structures, which then assembled with Monte Carlo simulations. We quantify the emergent entropic valence via a potential of mean force and torque. We generalize these shape operations to shape anisotropy dimensions, in analogy with the anisotropy dimensions introduced for enthalpically patchy particles. Our findings demonstrate that entropic patchiness and emergent valence provide a way of engineering directional bonding into nanoparticle systems, whether in the presence or absence of additional, non-entropic forces.

==> cube.tex <==
\begin{tikzpicture}[>=stealth']
  % set coordinates
  \coordinate (o) at (0,0);
  % these coordinates give an isometric projection
  %\coordinate (x) at ({1.7*cos(-150)},{1.7*sin(-150)});
  %\coordinate (y) at ({1.7*cos(-30)},{1.7*sin(-30)});
  % these coordinates given an anisometric projection
  \coordinate (x) at ({1.7*cos(-140)},{1.7*sin(-140)});
  \coordinate (y) at ({1.7*cos(-20)},{1.7*sin(-20)});
  \coordinate (z) at (0,1.7);
  % draw axes
  \coordinate (xc) at ($2.4*(x)$);
  \coordinate (yc) at ($2.4*(y)$);
  \coordinate (zc) at ($2.4*(z)$);
  % set the vertices for the cube
  \coordinate (vppp) at ($(o)+(x)+(y)+(z)$);
  \coordinate (vppm) at ($(o)+(x)+(y)-(z)$);
  \coordinate (vmpp) at ($(o)-(x)+(y)+(z)$);
  \coordinate (vmpm) at ($(o)-(x)+(y)-(z)$);
  \coordinate (vmmp) at ($(o)-(x)-(y)+(z)$);
  \coordinate (vmmm) at ($(o)-(x)-(y)-(z)$);
  \coordinate (vpmp) at ($(o)+(x)-(y)+(z)$);
  \coordinate (vpmm) at ($(o)+(x)-(y)-(z)$);
  % extra coordinates on top
  \coordinate (vpzp) at ($(o)+(x)+(z)$);
  \coordinate (vmzp) at ($(o)-(x)+(z)$);
  % make vertices in the cutting plane
  \coordinate (vppz) at ($(o)+(x)+(y)$);
  \coordinate (vmpz) at ($(o)-(x)+(y)$);
  \coordinate (vmmz) at ($(o)-(x)-(y)$);
  \coordinate (vpmz) at ($(o)+(x)-(y)$);
  % set the vertices for the cutting plane
  \coordinate (cppz) at ($(o)+1.15*(x)+1.15*(y)$);
  \coordinate (cmpz) at ($(o)-1.15*(x)+1.15*(y)$);
  \coordinate (cmmz) at ($(o)-1.15*(x)-1.15*(y)$);
  \coordinate (cpmz) at ($(o)+1.15*(x)-1.15*(y)$);
  % make vertices for the yz cutting plane
  \coordinate (Cmpp) at ($(o)-1.15*(x)+1.15*(y)+1.15*(z)$);
  \coordinate (Cmpm) at ($(o)-1.15*(x)+1.15*(y)-1.15*(z)$);
  \coordinate (Cmmp) at ($(o)-1.15*(x)-1.15*(y)+1.15*(z)$);
  \coordinate (Cmmm) at ($(o)-1.15*(x)-1.15*(y)-1.15*(z)$);
  % set the normals
  \coordinate (n1) at ($(o)+(x)$);
  \coordinate (n2) at ($(o)+(y)$);
  \coordinate (n3) at ($(o)+(z)$);
  \coordinate (n4) at ($(o)-(x)$);
  \coordinate (n5) at ($(o)-(y)$);
  \coordinate (n6) at ($(o)-(z)$);
  % set the face centres
  \coordinate (c1) at ($(n1)$);
  \coordinate (c2) at ($(n2)$);
  \coordinate (c3) at ($(n3)$);
  \coordinate (c4) at ($(n4)$);
  \coordinate (c5) at ($(n5)$);
  \coordinate (c6) at ($(n6)$);
  % draw the yz cutting plane
  \draw[fill=gcb9,opacity=0.6,draw=black,very thin,line join=round]
  (Cmpp) -- (Cmmp) -- (Cmmm) -- (Cmpm)--cycle;
  % draw the -xy face
  \draw[fill=gcb6,opacity=0.6,draw=black,very thin,line join=round]
  (vppm) -- (vmpm) -- (vmmm) -- (vpmm)--cycle;
  % draw rear bottom half faces
  \draw[fill=gcb6,opacity=0.6,draw=black,very thin,line join=round]
  (vmmm) -- (vmpm) -- (vmpz) -- (vmmz)--cycle;
  \draw[fill=gcb6,opacity=0.6,draw=black,very thin,line join=round]
  (vmmm) -- (vpmm) -- (vpmz) -- (vmmz)--cycle;
  % draw front bottom half faces
  \draw[fill=gcb6,opacity=0.6,draw=black,very thin,line join=round]
  (vppm) -- (vmpm) -- (vmpz) -- (vppz)--cycle;
  \draw[fill=gcb6,opacity=0.6,draw=black,very thin,line join=round]
  (vppm) -- (vpmm) -- (vpmz) -- (vppz)--cycle;
  % draw coordinate axes
  \draw[->] (o) -- (xc);
  \draw[->] (o) -- (yc);
  \node[draw=none,fill=none,left=0.2cm of xc](xl){$x$};
  \node[draw=none,fill=none,right=0.2cm of yc](yl){$y$};
  % draw cutting plane
  \draw[fill=gcb2,opacity=0.6,draw=black,very thin,line join=round]
  (cppz) -- (cmpz) -- (cmmz) -- (cpmz)--cycle;
  % draw rear top half faces
  \draw[fill=gcb6,opacity=0.6,draw=black,very thin,line join=round]
  (vmmp) -- (vmpp) -- (vmpz) -- (vmmz)--cycle;
  \draw[fill=gcb6,opacity=0.6,draw=black,very thin,line join=round]
  (vmmp) -- (vpmp) -- (vpmz) -- (vmmz)--cycle;
  % draw back half of top face
  \draw[fill=gcb6,opacity=0.6,draw=none]
  (vpzp) -- (vmzp) -- (vmmp) -- (vpmp)--cycle;
  % draw the z axis
  \draw[->] (o) -- (zc);
  \node[draw=none,fill=none,above=0.2cm of zc](zl){$z$};
  % draw front top half faces
  \draw[fill=gcb6,opacity=0.6,draw=black,very thin,line join=round]
  (vppp) -- (vmpp) -- (vmpz) -- (vppz)--cycle;
  \draw[fill=gcb6,opacity=0.6,draw=black,very thin,line join=round]
  (vppp) -- (vpmp) -- (vpmz) -- (vppz)--cycle;
  % draw front half of top face
  \draw[fill=gcb6,opacity=0.6,draw=none]
  (vppp) -- (vmpp) -- (vmzp) -- (vpzp)--cycle;
  % draw outline of top face
  \draw[fill=none,draw=black,very thin,line join=round]
  (vppp) -- (vmpp) -- (vmmp) -- (vpmp)--cycle;
\end{tikzpicture}


==> oct.tex <==
\begin{tikzpicture}[>=stealth']
  % set coordinates
  \coordinate (o) at (0,0);
  % these coordinates give an isometric projection
  %\coordinate (x) at ({2.3*cos(-150)},{2.3*sin(-150)});
  %\coordinate (y) at ({2.3*cos(-30)},{2.3*sin(-30)});
  % these coordinates given an anisometric projection
  \coordinate (x) at ({2.3*cos(-140)},{2.3*sin(-140)});
  \coordinate (y) at ({2.3*cos(-20)},{2.3*sin(-20)});
  \coordinate (z) at (0,2.3);
  % draw axes
  \coordinate (xc) at ($1.25*(x)$);
  \coordinate (yc) at ($1.25*(y)$);
  \coordinate (zc) at ($1.25*(z)$);
  % set the vertices for the octahedron
  \coordinate (vpzz) at ($(o)+(x)$);
  \coordinate (vzpz) at ($(o)+(y)$);
  \coordinate (vzzp) at ($(o)+(z)$);
  \coordinate (vmzz) at ($(o)-(x)$);
  \coordinate (vzmz) at ($(o)-(y)$);
  \coordinate (vzzm) at ($(o)-(z)$);
  % make vertices in the cutting plane
  \coordinate (vpz3) at ($(o)+(x)-0.333333*(x)+0.333333*(z)$);
  \coordinate (vzp3) at ($(o)+(y)-0.333333*(y)+0.333333*(z)$);
  \coordinate (vmz3) at ($(o)-(x)+0.333333*(x)+0.333333*(z)$);
  \coordinate (vzm3) at ($(o)-(y)+0.333333*(y)+0.333333*(z)$);
  % set the vertices for the cutting plane
  \coordinate (cpz3) at ($(o)+1.15*(x)-0.333333*(x)+0.333333*(z)$);
  \coordinate (czp3) at ($(o)+1.15*(y)-0.333333*(y)+0.333333*(z)$);
  \coordinate (cmz3) at ($(o)-1.15*(x)+0.333333*(x)+0.333333*(z)$);
  \coordinate (czm3) at ($(o)-1.15*(y)+0.333333*(y)+0.333333*(z)$);
  % make vertices for the yz cutting plane
  \coordinate (Cmzz) at ($(o)-1.15*(x)$);
  \coordinate (Czpz) at ($(o)+1.15*(y)$);
  \coordinate (Czzp) at ($(o)+1.15*(z)$);
  % draw the bottom faces
  \draw[fill=gcb2,opacity=0.6,draw=black,very thin,line join=round]
  (vmzz) -- (vzmz) -- (vzzm)--cycle;
  \draw[fill=gcb2,opacity=0.6,draw=black,very thin,line join=round]
  (vmzz) -- (vzpz) -- (vzzm)--cycle;
  \draw[fill=gcb2,opacity=0.6,draw=black,very thin,line join=round]
  (vpzz) -- (vzmz) -- (vzzm)--cycle;
  \draw[fill=gcb2,opacity=0.6,draw=black,very thin,line join=round]
  (vpzz) -- (vzpz) -- (vzzm)--cycle;
  % draw coordinate axes
  \draw[->] (o) -- (xc);
  \draw[->] (o) -- (yc);
  \node[draw=none,fill=none,left=0.2cm of xc](xl){$x$};
  \node[draw=none,fill=none,right=0.2cm of yc](yl){$y$};
  % draw top faces below cutting plane
  \draw[fill=gcb2,opacity=0.6,draw=black,very thin,line join=round]
  (vmzz) -- (vzmz) -- (vzm3) -- (vmz3)--cycle;
  \draw[fill=gcb2,opacity=0.6,draw=black,very thin,line join=round]
  (vmzz) -- (vzpz) -- (vzp3) -- (vmz3)--cycle;
  \draw[fill=gcb2,opacity=0.6,draw=black,very thin,line join=round]
  (vpzz) -- (vzmz) -- (vzm3) -- (vpz3)--cycle;
  \draw[fill=gcb2,opacity=0.6,draw=black,very thin,line join=round]
  (vpzz) -- (vzpz) -- (vzp3) -- (vpz3)--cycle;
  % draw cutting plane
  \draw[fill=gcb6,opacity=0.6,draw=black,very thin,line join=round]
  (cpz3) -- (czp3) -- (cmz3) -- (czm3)--cycle;
  % draw top part of faces
  \draw[fill=gcb2,opacity=0.6,draw=black,very thin,line join=round]
  (vzm3) -- (vmz3) -- (vzzp)--cycle;
  % draw the z axis
  \draw[->] (o) -- (zc);
  \node[draw=none,fill=none,above=0.2cm of zc](zl){$z$};
  % draw remaining top half of faces
  \draw[fill=gcb2,opacity=0.6,draw=black,very thin,line join=round]
  (vzp3) -- (vmz3) -- (vzzp)--cycle;
  \draw[fill=gcb2,opacity=0.6,draw=black,very thin,line join=round]
  (vzm3) -- (vpz3) -- (vzzp)--cycle;
  \draw[fill=gcb2,opacity=0.6,draw=black,very thin,line join=round]
  (vzp3) -- (vpz3) -- (vzzp)--cycle;
  % draw the yz cutting plane
  \draw[fill=gcb9,opacity=0.6,draw=black,very thin,line join=round]
  (Cmzz) -- (Czpz) -- (Czzp)--cycle;
\end{tikzpicture}


==> tet.tex <==
\begin{tikzpicture}[>=stealth']
  % set coordinates
  \coordinate (o) at (0,0);
  % these coordinates give an isometric projection
  %\coordinate (x) at ({1.7*cos(-150)},{1.7*sin(-150)});
  %\coordinate (y) at ({1.7*cos(-30)},{1.7*sin(-30)});
  % these coordinates given an anisometric projection
  \coordinate (x) at ({1.7*cos(-140)},{1.7*sin(-140)});
  \coordinate (y) at ({1.7*cos(-20)},{1.7*sin(-20)});
  \coordinate (z) at (0,1.7);
  % draw axes
  \coordinate (xc) at ($2.25*(x)$);
  \coordinate (yc) at ($2.25*(y)$);
  \coordinate (zc) at ($2.25*(z)$);
  % set the vertices for the tetrahedron
  \coordinate (vppp) at ($(o)+{sqrt(2)}*(x)+(z)$);
  \coordinate (vmmp) at ($(o)-{sqrt(2)}*(x)+(z)$);
  \coordinate (vpmm) at ($(o)+{sqrt(2)}*(y)-(z)$);
  \coordinate (vmpm) at ($(o)-{sqrt(2)}*(y)-(z)$);
  % make vertices in the cutting plane
  \coordinate (vzzp) at ($(o)+(z)$);
  % make vertices for the yz cutting plane
  \coordinate (Czpm) at ($(o)+{1.15*sqrt(2)}*(y)-1.15*(z)$);
  \coordinate (Czmm) at ($(o)-{1.15*sqrt(2)}*(y)-1.15*(z)$);
  \coordinate (Czzp) at ($(o)+1.15*(z)$);
  % one additional vertex for the parallel cutting plane
  \coordinate (Cmzp) at ($(o)-{1.15*sqrt(2)}*(x)+1.15*(z)$);
  % draw the bottom faces
  % draw coordinate axes
  \draw[->] (o) -- (xc);
  \draw[->] (o) -- (yc);
  \node[draw=none,fill=none,left=0.2cm of xc](xl){$x$};
  \node[draw=none,fill=none,right=0.2cm of yc](yl){$y$};
  % draw the z axis
  \draw[->] (o) -- (zc);
  \node[draw=none,fill=none,above=0.2cm of zc](zl){$z$};
  % the parallel cutting plane
  \draw[fill=gcb1,opacity=0.6,draw=black,very thin,line join=round]
  (Czpm) -- (Czmm) -- (Cmzp)--cycle;
  % draw top faces below cutting plane
  \draw[fill=gcb4,opacity=0.6,draw=black,very thin,line join=round]
  (vmpm) -- (vpmm) -- (vmmp)--cycle;
  \draw[fill=gcb4,opacity=0.6,draw=black,very thin,line join=round]
  (vzzp) -- (vmmp) -- (vmpm)--cycle;
  \draw[fill=gcb4,opacity=0.6,draw=black,very thin,line join=round]
  (vzzp) -- (vmmp) -- (vpmm)--cycle;
  % cutting plane goes here
  \draw[fill=gcb9,opacity=0.6,draw=black,very thin,line join=round]
  (Czpm) -- (Czmm) -- (Czzp)--cycle;
  % draw things in front of the cutting plane
  \draw[fill=gcb4,opacity=0.6,draw=black,very thin,line join=round]
  (vzzp) -- (vppp) -- (vmpm)--cycle;
  \draw[fill=gcb4,opacity=0.6,draw=black,very thin,line join=round]
  (vmpm) -- (vpmm) -- (vppp)--cycle;
  \draw[fill=gcb4,opacity=0.6,draw=black,very thin,line join=round]
  (vzzp) -- (vppp) -- (vpmm)--cycle;
\end{tikzpicture}

